Distance Measures for Embedded Graphs

We introduce new distance measures for comparing straight-line embedded graphs based on the Fr\'echet distance and the weak Fr\'echet distance. These graph distances are defined using continuous mappings and thus take the combinatorial structure as well as the geometric embeddings of the graphs into account. We present a general algorithmic approach for computing these graph distances. Although we show that deciding the distances is NP-hard for general embedded graphs, we prove that our approach yields polynomial time algorithms if the graphs are trees, and for the distance based on the weak Fr\'echet distance if the graphs are planar embedded. Moreover, we prove that deciding the distances based on the Fr\'echet distance remains NP-hard for planar embedded graphs and show how our general algorithmic approach yields an exponential time algorithm and a polynomial time approximation algorithm for this case.

==> body/algorithmsPlaneGraphs.tex <==
\subsection{Exponential Time Algorithm}
\label{sec:exponential_time_algo_details}
Here, we give some more details on the implementation of the idea
presented in Section~\ref{sec:exponential_time_algo}.
\begin{figure}[b]
\centering
\includegraphics[page=1, width=0.7\textwidth]{plane-decomposition}
\caption{A plane graph (a) is recursively decomposed into chordless cycles by splitting each cycle with a chord (b).}
\label{fig:gd-plane-decomposition}
\end{figure}

First, we remove all tree-like substructures of $G_1$ and map these as
described in the proof of Lemma~\ref{lem:gd-map-tree}. Next, we
decompose the remainder of $G_1$ into chordless cycles, where a chord
is a maximal path in $G_1$ incident to two faces, see
Figure~\ref{fig:gd-plane-decomposition}. We map the parts of $G_1$
from bottom up, deciding in each step if we can map two adjacent
cycles and all the nested substructures of the cycles
simultaneously. To do so, we start with storing all combinations of
placements of endpoints of a chord -which separates two faces
(chordless cycles)- allowing us to map the two faces
simultaneously. We prune all placements which are not part of any
valid combination. In the following steps, for each placement $C_u$ of
an endpoint $u$ of a chord and each valid combination $c$ of nested
chords computed in the previous step, we run one graph
exploration. For each placement $C_v$ of the other endpoint $v$ of the
chord, which allow to map both cycles simultaneously, we store a new
combination consisting of $C_u$, $c$ and $C_v$. We prune all
placements of $u$ where we cannot reach a valid placement of $v$ by
using any of the previous computed combinations. Furthermore, we prune
those placements of $v$ which are never reached by any graph
exploration. If the list of placements gets empty for one vertex, we
can conclude, that the graph distance is greater than
$\eps$. Conversely, if we find a valid combination of placements of
the endpoints of the chord in the last step, we can conclude that we
can map the whole graph $G_1$ as we guarantee in each step that all
substructures can be mapped, too.

\paragraph*{Proof of \thmref{thm:exponential_time}}
Each graph exploration takes $O(m_2)$ time and in each node we have to
run $O(m_2k)$ explorations, where $k$ is the number of valid
combinations of endpoint placements from previously investigated
chords. As the tree has a depth of $\log(F)$, we have
\begin{ceqn}
\begin{align*}
 \frac{F}{2} m_2^2 + \frac{F}{4} m_2^2m_2^4 + \dots + m_2^2\left(m_2^{2^{log(F)-2}}\right)^2
 = F \sum_{i=1}^{\log(F)} \frac{1}{2^i} m_2^{2^{i+1}-2}
\end{align*}
\end{ceqn}
as the total running time of the graph explorations. We can upper bound this term as follows:
\begin{ceqn}
\begin{align*}
&F \sum_{i=1}^{\log(F)} \frac{1}{2^i} m_2^{2^{i+1}-2}
\leq F \sum_{i=1}^{\log(F)} m_2^{2^{i+1}-2}
\leq F \sum_{i=1}^{2^{\log(F)+1}-2} m_2^{i}\\
&= F \sum_{i=1}^{2F-2} m_2^{i}
= F \frac{m_2^{2F-1}-m_2}{m_2-1} \in O\left(F m_2^{2F-1}\right),
\end{align*}
\end{ceqn}
where the second equality uses
\begin{ceqn}
\begin{align*}
\sum_{i=1}^n a^i = \frac{a(a^n - 1)}{a-1},
\end{align*}
\end{ceqn}

for $a \in \mathbb{R}$.  In the first step, we have to store
$O(m_2^2)$ combinations for each two faces we want to map
simultaneously.  Let $k$ be the number of combinations in the previous
step. Then we have to store up to $k^2m_2^2$ combinations in the next
step. This results in storing $O(m_2^{2F-1})$ combinations in the root
node of the decomposition.

\subsection{Proof of \thmref{thm:alpha-approximation}}
\begin{figure}[t]
\centering
\includegraphics[scale=0.6]{alpha-approximation}
\caption{Illustration of the proof of
  Theorem~\ref{thm:alpha-approximation}. (a) Three valid
  $\eps$-placements form one connected component inside a slightly
  larger ball around $v$. (b) In case of short edges, the placements
  remain unconnected also inside a larger surrounding of $v$. }
\label{fig:alpha-approximation}
\end{figure}
Let $\alpha$ be the smallest angle between two edges incident to a
vertex $v$ with degree at least three and let $C_1,C_2,\dots, C_j$ be
the valid placements of $v$ for a given distance value
$\eps$. Furthermore, let $V_{C_i}$ be the set of vertices of $C_i$. It
can be easily shown that for a larger distance value of $\hat{\eps}
\geq \frac{1}{\sin(\alpha)}\eps$ there exists vertices $v_1,v_2,\dots,
v_k$, embedded inside $B_{\hat{\eps} }$, such that the subgraph $C =
(V',E')$, where $V' = \bigcup\limits_{i=1}^{j} V_{C_i} \cup \{v_1\}
\cup \{v_2\} \cup \dots \cup \{v_k\}$ and $E'=\{\{uw\} \in E_2| u \in
V', w \in V'\}$ is connected, see
Figure~\ref{fig:alpha-approximation}~(a). Note that this property is
not true if $B_\eps(v_1) \cap B_\eps(v_2) \neq \emptyset$ for two
adjacent vertices $v_1$, $v_2 \in V_1$:
Figure~\ref{fig:alpha-approximation}~(b) shows an example with
$\alpha=45^\circ$ where the two placements do not merge inside
$B_{\frac{\varepsilon}{\sin(45^\circ)}}(v)$. However, with the
condition $B_\eps(v_1) \cap B_\eps(v_2) = \emptyset$, there is only
one valid $\frac{1}{\sin(\alpha)} \eps$-placement $C$ for each vertex
with degree at least three. Furthermore, every valid $\eps$ placement
is a valid $\frac{1}{\sin(\alpha)} \eps$-placement. Now, a path $P$ of
$G_1$ starting at a vertex $v$ with $deg(v)\geq 3$ and ending at a
vertex $w$ with $deg(w)\neq 2$, with vertices of degree two in the
interior of $P$, can be mapped as described in the proof of
Lemma~\ref{lem:gd-map-tree} . For two paths which start and/or end at
a common vertex $v$, $v$ is mapped to the same placement as there is
only one valid $\frac{1}{\sin(\alpha)} \eps$-placement of $v$. This
ensures that each edge of $G_1$ is mapped correctly.


==> body/hardnessGeneralGraphs.tex <==
We show NP-hardness with a reduction from binary constraint
satisfaction problem (CSP), which is defined as follows:

\begin{problem}
\proc{Binary Constraint Satisfaction Problem (CSP)}\\
\noindent \textbf{Instance:} A set of variables
$X=\{x_1,\ldots,x_n\}$, variable domains \\ $D = \{D_1,\ldots,D_n\}$
and a set of constraints $C = \{C_1,\ldots,C_m\}$, where each
constraint $C$ has two variables $x_i$, $x_j$ and a relation $R_C
\subseteq D_i\times D_j$.\\
\noindent \textbf{Question:} Can each variable $x_i$ be assigned a
value $d_i\in D_i$ such that for each constraint $C$ on variables
$x_i$, $x_j$, their values $(d_i,d_j)$ satisfy $R_C$?
\end{problem}

Consider an instance $\langle X, D, C\rangle$.  Set $\eps=1$.  Every
variable $x_i$ is represented by a vertex $v_i$ in $G_1$ and for each
constraint $C_k$ on variables $x_i$, $x_j$, $G_1$ has an edge
$\{v_i,v_j\}$ in $G_1$.  We embed $G_1$ such that all adjacent
$\eps$-balls are separated by at least $2\eps$ and no $\eps$-tube of
an edge overlaps an $\eps$-ball that does not belong to one of the
edge's endpoints.  This can for example be realized by placing all
vertices on a sufficiently large circle.

Every value $d_{i,a}\in D_i$ is represented by a vertex $u_{i,a}$ in
$G_2$ that is inside the $\eps$-ball of $v_i$.  For each pair of
values $d_{i,a}\in D_i$, $d_{j,b}\in D_j$ allowed by a constraint on
$x_i$ and $x_j$, $G_2$ has an edge $\{u_{i,a},u_{j,b}\}$.  This way,
every vertex $u_{i,a}$ of $G_2$ defines exactly one $\eps$-placement
of the corresponding vertex $v_i$ in $G_1$.
Figure~\ref{fig:csp-reduction} illustrates the construction.
\begin{figure}[b]
\centering
\includegraphics[width=.5\textwidth]{reduction_bcsp}
\caption{Illustration of the reduction from BCSP.}
\label{fig:csp-reduction}
\end{figure}

A solution to the CSP consists of selecting a value $d_i\in D_i$ for
each variable $x_i$, such that if there is a constraint on $v_i$ and
$v_j$, the pair $\{d_i,d_j\}$ satisfies the constraint.  This is
equivalent to selecting a placement $d_i$ of each vertex $v_i$, such
that if $G_1$ has an edge $\{v_i,v_j\}$, then $G_2$ has an edge
connecting $u_i$, $u_j$ representing $d_i$ and $d_j$, respectively.
The graph distance problem has the weaker requirement that there
exists a path $P_{i,j}$ between $u_i$ and $u_j$, such that
$\delta_F(\{v_i,v_j\},P_{i,j})\leq\eps$.  However, the construction is
such that only paths consisting of a single edge are permitted for the
strong distance, since $\eps$-balls must be sufficiently separated and
nonoverlapping with $\eps$-tubes.  So $G_2$ must have an edge
$\{u_i,u_j\}$ if $G_1$ has an edge $\{v_i,v_j\}$.  So,
$\distDir(G_1,G_2)\leq\eps$ if and only if $\langle X,D,C \rangle$ is
a satisfiable binary CSP.

For the weak graph distance, edges in $G_1$ can be mapped to paths
consisting of multiple edges in $G_2$.  In this case, there may be
weak placements of $G_1$ that do not represent a solution to the
constraint satisfaction instance.  To remedy this, we insert a vertex
in the middle of each edge of $G_1$.  The vertex is placed such that
its $\eps$-ball is separated from the $\eps$-balls of the original
endpoints of the edge by at least $2\eps$, so each of the new edges is
mapped to part of a single edge in $G_2$.  In this construction
$\distDirWeak(G_1,G_2)\leq\eps$ if and only if $\langle X,D,C \rangle$
is a satisfiable binary CSP.


==> body/hardnessPlaneGraphs.tex <==
\begin{figure}
\centering
\includegraphics[width=.7\textwidth]{plane-valid-counterexample}
\caption{An example of plane graphs $G_1$ (blue) and $G_2$ (red) where
  every vertex of $G_1$ has two valid placements, but there is no
  $\eps$-placement of $G_1$: If the central edge $e$ is mapped to a
  path through $e_1$, there is no way to map the cycle bounding face
  $F_2$ on the right, and if $e$ is mapped to a path through $e_2$,
  the cycle bounding $F_1$ cannot be mapped.}
\label{fig:plane-valid-counterexample}
\end{figure}


\subsection{Proof of \thmref{theorem:NP_plane}}
We prove the NP-hardness by a reduction from
\textsc{Monotone-Planar-3-Sat}. In this \textsc{3-Sat} variant, the
associated graph with edges between variables and clauses is planar
and each clause contains only positive or only negative literals. The
overall idea is to construct two graphs $G_1$ and $G_2$ based on a
\textsc{Monotone-Planar-3-Sat} instance $A$, such that $A$ is
satisfiable if and only if $\distDir(G_1,G_2) \leq\eps$. That is, we
construct subgraphs of $G_1$ and $G_2$, where some edges of $G_2$ are
labeled \textsc{True} or \textsc{False} in a way, such that only
certain combinations of \textsc{True} and \textsc{False} values can be
realized by a placement of $G_1$ to $G_2$.  To realize other
combinations, backtracking, at least along one edge of $G_1$, is
necessary. But this is not allowed for the strong graph distance.  In
the following, we describe the construction of the gadgets (subgraphs)
for the variables and the clauses of a \textsc{Monotone-Planar-3-Sat}
instance. Additionally, we need a gadget to split a variable if it is
contained in several clauses and a gadget which connects the variable
gadgets with the clause gadgets. Furthermore, we prove for each gadget
which \textsc{True} and \textsc{False} combinations can be realized
and which combinations are not possible.  All constructed edges are
straight line edges. The graph $G_1$ is shown in blue color and $G_2$
is shown in red color in the sketches used to illustrate the ideas of
the proof. We denote $T_{\eps}(e)$ as the $\eps$-tube around the edge
$e$. All vertices of the graph can be either mapped arbitrarily within
a given $\eps$-surrounding and with a given minimal distance from each
other or must lie at the intersection of two lines. Thus, we can
ensure that the construction uses rational coordinates only and can be
computed in polynomial time.

Following a reparameterization of an edge or a path (embedded curve)
as described in Definition \ref{def:distances}, we denote by the term
"walking along an edge or a path". In this sense backtracking means
that the reparametization is not injective and thus, if backtracking
is necessary to stay within $\eps$-distance to another path or edge
one can conclude that the \fr distance between these paths or edges is
greater than $\eps$ as in this case it is required that the
reparameterization is injective.

Furthermore, we call a path labeled \textsc{True} (\textsc{False})
shortly a \textsc{True} (\textsc{False}) signal.


\begin{figure}
\centering
\includegraphics[scale=0.745]{gadgets_all}
\caption{Building blocks to build graph-similarity instance given a \textsc{Monotone-Planar-3-Sat} instance.}
\label{fig:gadgets}
\end{figure}

In the following, we give a detailed description of the construction
and the properties of the gadgets.  The \textsc{Variable} gadget: For
each variable of $A$, we add a vertex $v$ and two edges, $e_1$ and
$e_2$, of $G_1$ incident to a vertex $v$, where the angle between
$e_1$ and $e_2$ is between $90^{\circ}$ and $120^{\circ}$. We add a
vertex $w_1$ ($w_2$) of $G_2$ on the intersection of the outer
boundaries of $T_{\eps}(e_2)$ ($T_{\eps}(e_1)$) and a line through
$e_1$ ($e_2$). Furthermore, we add a vertex $w_3$ of $G_2$ at the
intersection of the boundaries of $T_{\eps}(e_1)$ and
$T_{\eps}(e_2)$. See the upper left sketch in Figure \ref{fig:gadgets}
for an illustration. We connect $w_1$ and $w_2$ with $w_3$ and draw an
edge from $w_1$ and $w_2$ inside the $\eps$-tubes around $e_1$ and
$e_2$, with labels \textsc{True}. Analogously, we embed two edges from
$w_3$ with the label \textsc{False}. For the \textsc{Variable} gadget
a \textsc{True}-\textsc{True} combination is not possible: There are
two placements $p_1$ and $p_2$ of the vertex $v$. Assume we choose
$p_1$. Note that one can map $e_1$ to a path containing the edge of
$G_2$ with the \textsc{True} labeling inside $T_\eps(e_1)$. Now, we
want to map $e_2$ to a path $P$ starting at some point of $p_1$, where
$P$ contains the edge of $G_2$ with the \textsc{True} labeling inside
$T_\eps(e_2)$. In this case, one has to walk along $e_2$ up to $q$
(the point on $e_2$ with distance $\eps$ to $w_3$) while walking
simultaneously to $w_3$ on $P$. But then, when walking along $P$ up to
$w_1$, one must walk back along $e_2$ up to $v$ as any point along the
interior of $e_1$ has distance greater than $\eps$ to $w_1$. Thus,
$\delta_F(e_2, P) > \eps$. It is easy to see that for any other
combination of labels there is a placement $p$ of $v$, such that $e_1$
and $e_2$ can be mapped to a path $P_1$ ($P_2$) starting at a point
$a$ of $p$ with $\delta_F(e_2, P_1) \leq \eps$ ($\delta_F(e_2, P_2)
\leq \eps$).

A \textsc{Permute} gadget is the same as the \textsc{Variable} gadget, but with a different labeling, see Figure \ref{fig:gadgets}.
The construction of the \textsc{Split} gadget is similar to the \textsc{Variable} gadget. Additionally, we add a third edge $e_3$ of $G_1$ and edges of $G_2$ from $w_2$ and $w_3$ inside the $\eps$-tube around $e_3$. For the labeling, see Figure~\ref{fig:gadgets}.

The same argument as for the \textsc{Variable} gadget is used to proof
the following statements:
\begin{itemize}
\item A \textsc{False} signal can never be converted to a \textsc{True} signal in the \textsc{Split} gadget.
\item A \textsc{False} signal can never be converted to a \textsc{True} signal in the \textsc{Permute} gadget.
\end{itemize}

Furthermore, a \textsc{True} signal can, but need not to be converted
to a \textsc{False} signal in the \textsc{Permute} gadget.

We construct the \textsc{Wire} gadget used to connect all the other
gadgets by drawing two edges $e_1$ and $e_2$ of $G_1$ incident to a
vertex $v$ (with arbitrary angle) and two vertices $w_1$ and $w_2$ of
$G_2$ inside $B_{\eps}(v)$ with non intersecting incident edges inside
$T_{\eps}(e_1)$ and $T_{\eps}(e_2)$. Obviously, it is not possible to
convert a \textsc{True} signal to a \textsc{False} signal or vice
versa, here.

For the \textsc{Clause} gadget, we first introduce a
\textsc{NAE-Clause} gadget. Here it is required that the three values
in each clause are not all equal to each other. We start the
construction of the \textsc{NAE-Clause} gadget by drawing three edges
$e_1$, $e_2$ and $e_3$ incident to a vertex $v$ with a pairwise
$120^{\circ}$ angle. We draw three vertices $w_1$, $w_2$ and $w_3$ on
the intersections of $T_{\eps}(e_1)$, $T_{\eps}(e_2)$ and
$T_{\eps}(e_3)$ with a maximum distance to $v$. Furthermore, we draw
two edges of $G_2$ inside the tubes for each vertex and label them as
shown in Figure~\ref{fig:gadgets}. Let $q_1$ be the point on $e_1$
with distance $\eps$ to $w_1$ and $w_2$. Here, it is not enough to
simply connect $w_1$ and $w_2$ with one edge as shown in the bottom
left sketch of Figure~\ref{fig:gadgets}. To force backtracking along
$e_1$ for a combination of labels which we want to exclude, we have to
ensure that a path from $w_1$ to $w_2$ leaves $B_\eps(q_1)$ but stays,
once entered, inside $B_\eps(v)$. For the other pairs, $(w_1, w_3)$
and $(w_2, w_3)$ we do the same. A possible drawing of these paths
maintaining the planarity of $G_2$ is shown in \figref{fig:gadgets}.
The three placements of $v$ are connected by the vertices $w_1$, $w_2$
and $w_3$ and it holds that there is no placement of $v$ such that an
all-\textsc{False} or an all-\textsc{True} labeling can be realized:
Suppose we map $v$ to $s(v)$ as shown in the
\figref{fig:gadgets}. Then, edges $e_2$ and $e_3$ can be mapped to
paths through edges labeled \textsc{True}. But we cannot map $e_1$ to
such a path $P$: When $P$ reaches vertex $w_1$, any corresponding
reparameterization of $e_1$ realizing $\delta_F(e_1,P)\leq\eps$ must
have reached $q_1$ as $q_1$ is the only point with distance at most
$\eps$ to $w_1$ on $e_2$. As $P$ leaves $B_\eps(q_1)$ between $w_1$
and $w_2$ and any point on $e_1$ with distance at most $\eps$ to the
part of $P$ outside $B_\eps(q_1)$ lies between $v$ and $q_1$ it
follows that $\delta_F(e_1,P)>\eps$. For symmetric reasons it follows
that any other all-equal labeling cannot be realized. However, there
is a placement of $v$, such that all three edges $e_1$, $e_2$ and
$e_3$ can be mapped to a path in $G_2$ with \fr\ at most $\eps$, for
each configuration where not all three signals have the same value.

\textsc{Monotone-Planar-NAE-3-Sat} is in $P$, but we can use the
\textsc{NAE-Clause} gadget as core of our \textsc{Clause} gadget
referring to the NP-complete version \textsc{Monotone-Planar-3-Sat}:
We obtain the \textsc{Clause} gadget by connecting each
\textsc{NAE-Clause} gadget with three \textsc{Permute} gadgets, as
shown in Figure~\ref{fig:gadgets}.

\figref{fig:graph_construction} partially shows the constructed graphs for a given \textsc{Monotone-Planar-3-Sat} $A$ consisting of the subgraphs (gadgets) described above.

\begin{figure}
\centering
\includegraphics[scale=0.745]{graph_construction_new}
\caption{For the \textsc{Monotone-Planar-3-Sat} instance $A$ with
  variables $V=\{x_1,x_2,\dots,x_5\}$ and clauses $C=\{(x_1 \vee x_2
  \vee x_3), (x_3 \vee x_4 \vee x_5), (\bar{x_1} \vee \bar{x_3} \vee
  \bar{x_5})\}$ the Figure shows the construction of the clause $(x_1
  \vee x_2 \vee x_3)$.}
\label{fig:graph_construction}
\end{figure}

Now, given a \textsc{Monotone-Planar-3-SAT} instance $A$, one can
construct the graphs $G_1$ and $G_2$ with the gadgets described
above. Note that all gadgets are plane subgraphs. By placing them next
to each other with no overlap, we can ensure that $G_1$ and $G_2$ are
plane graphs.

A valid placement of the whole graph $G_1$ induces a solution of $A$:
In the corresponding gadget for each positive NAE-clauses, at least
one of the outgoing edges of $G_1$ must be mapped to a path through an
edge labeled \textsc{True}. By construction, this label cannot be
converted to \textsc{False} in any of the gadgets and therefore the
corresponding variable $v$ gets the value \textsc{True}. In this case,
$v$ cannot set any of the negative clauses \textsc{True} because the
other outgoing edge must be mapped to a path through the edge of $G_2$
labeled \textsc{False} and this signal can never be switched to
\textsc{True}. The same holds for the case of negative NAE-clauses.

Conversely, given a solution $S$ of the \textsc{Monotone-Planar-3-SAT}
instance $A$, it is easy to construct a placement of $G_1$. In the
variable gadget of variable $x_1$, we chose placement $p_1$ and map
$e_1$ to a path through the edge of $G_2$, labeled \textsc{True} and
map $e_2$ to a path through the edge labeled \textsc{False} if $x_1$
is positive in $S$. If $x_1$ is negative, we chose placement $p_2$ and
map $e_1$ and $e_2$ accordingly.  All edges of the other gadget now
can be mapped to $G_2$ in a signal preserving manner (\textsc{True}
stays \textsc{True}, \textsc{False} stays \textsc{False}). If there
exists a clause $C$ in $A$, such that all three variables of $C$ are
positive (negative) in $S$, we change one signal in the
\textsc{Permute} gadget from \textsc{True} to \textsc{False}. Thus, we
have found a placement for the whole graph $G_1$.

\subsection{Proof of \thmref{thm:c_hard}}
\begin{figure}
\centering
\includegraphics[scale=0.65]{approximation}
\caption{Illustration of the proof of Theorem~\ref{thm:c_hard}.}
\label{fig:approximation}
\end{figure}
The theorem follows from the observation that we can grow $\eps$ a
certain amount, preserving the characteristics of the gadgets. We give
a detailed proof for the \textsc{NAE-Clause} gadget and note that a
similar argument holds for the other gadgets. See
Figure~\ref{fig:approximation} for an illustration of the arguments
and the calculations below.

Let us fix $\eps = 1$. As described in the proof of
Theorem~\ref{theorem:NP_plane}, we connect the vertices $w_1$ and
$w_2$ by a path which leaves $B_{1}(q_1)$, but stays inside
$B_{1}(v_1)$. (Introducing a spike which leaves $B_{1}(q_1)$ and
returns to $B_{1}(q_1)$, see Figure~\ref{fig:gadgets}). We draw the
spike such that its peak is arbitrarily close to the intersection of a
straight line through the edge $e_1$ and the $1$-circle around
$v$. When enlarging $\eps$, the point $q_1$ moves along $e_1$ toward
$v$. We need to compute the smallest value $\delta_{min}$, such that
$B_{1}(v)$ is completely contained in $B_{1+\delta_{min}}(q_1)$. For
any value $\delta < \delta_{min}$, there exists a drawing of the
spikes, such that the characteristics of the \textsc{NAE-Clause}
gadget still hold, e.g., there is no placement of $v$ allowing an
all-equal-labeling.

Note that $\delta_{min}$ equals the distance from $q_1$ to $v$, when
$q_1$ is at distance $1+\delta_{min}$ to $w_1$. Let $q'$ be the
position of $q_1$ for $\delta=0$ and let $d$ be the distance between
$q'$ and $q_1$. Then we have
$%\begin{equation*}
\tan(30^{\circ}) = \frac{\delta_{min} + d}{1} =\delta_{min} + d
$. %\end{equation*}
Furthermore, we have
$%\begin{equation*}
d = \sqrt{(1+\delta_{min})^2 -1}
$ %\end{equation*}
and therefore
$%\begin{equation}
\delta_{min} = \tan(30^{\circ}) - \sqrt{(1+\delta_{min})^2 -1}
%\label{eq:delta}
$, %\end{equation}
which solves to
%Solving~\ref{eq:delta}, we obtain
$\delta_{min} = \frac{1}{4} - \frac{1}{4\sqrt{3}} \approx 0.10566 $.
The factor by which $\eps$ can be multiplied is greater than
$1+\delta_{min}$ for all other gadgets. Thus, $\delta_{min}$ is the
critical value for the whole construction and the theorem follows.


==> body/proofOfLemmas.tex <==
\subsection{\lemref{lem:unique-valid-pl}}
Map each internal vertex $v$ to a point $s(v)$ on %the representative
of its unique (weakly) valid placement $C_v$. %: $s(v) = r(C_v)$.
Consider an edge $e=\{u,v\}\in E_1$.  In the previous step, at least
one (weak) placement $P_e$ of $e$ was discovered that connects points
$p_0$ and $p_k$ on $C_u$ and $C_v$, respectively, since otherwise
$C_u$ and $C_v$ would be invalid.  If $p_k \neq s(v)$, $P_e$ can be
adapted by shortening it and/or concatenating a path on $C_v$
(i.e.\ inside $B_\eps(v)$) without causing its (weak) \fr to $e$ to
become $>\eps$.  Adapt $P_e$ to a path $P'_e$ that has endpoints
$p'_0=s(u)$ and $p'_k=s(v)$ and define $s(e)=P'_e$.  Now, $s$ is a
graph mapping from $G_1$ to $G_2$ and each edge is mapped to a path
with (weak) \fr at most $\eps$, so $\distDir(G_1,G_2)\leq\eps$ (or
$\distDirWeak(G_1,G_2)\leq\eps$). Recall, that each vertex $w$ of
degree one is either connected to an internal vertex $i$, or $G_1$
consists of only one edge $\{w,x\}$. The first case is already
covered, since the unique valid (weak) placement $C_i$ for $i$ is
reachable from any valid (weak) placement of $w$. The latter case
follows because every vertex placement for $w$ is valid, i.e., for
each placement $C_w$ for $w$ there is a (weakly) reachable placement
$C_x$ for $x$ and any combination of two reachable placements $C_w$
and $C_x$ yields a valid (weak) placement of $G_1$.

\subsection{\lemref{lem:gd-map-tree}}
We view $G_1$ as a rooted tree, selecting an arbitrary vertex as the
root.  We map all vertices of $G_1$ from the root outwards.  First,
map the root to an arbitrary (weakly) valid placement.  When
processing a vertex $v$: Map $v$ to an arbitrary (weakly) valid
placement that is reachable from the placement its parent $p$ is
mapped to.  Recall, that a (weak) $\eps$-placement of a vertex is
\emph{(weakly) valid} if there is an $\eps$-placement for every
incident edge. Since $p$ was mapped to a (weakly) valid placement and
there is an edge $\{p,v\}$ in $G_1$, there must be at least one such
placement of $v$ by definition of a (weakly) valid placement.  Since
all edges in $G_1$ are tree edges, this ensures that every edge is
mapped correctly, that is to a path with (weak) \fr\ at most $\eps$.

\begin{notation}
In the following proofs, we use the expression "map" $G_S$ to denote
mapping a subgraph $G_S$ of $G_1$ to $G_2$ such that the mapping
realizes $\distDir(G_S, G_2) \leq \eps$.
\end{notation}

\subsection{\lemref{lem:gd-weak-plane}}
%\begin{proof}
A \emph{tree-substructure} of $G_1$ is a tree $T = (V_T, E_T)$ induced
by the vertex set $V_T \subset V_1$ with a root vertex $r \in V_T$,
such that for all vertices $v\in V_T$, $v \neq r$, $v$ is not an
endpoint of an edge $e \in E_1 \backslash E_T$ and such that $T$ is
maximal, in the sense that when adding one additional vertex, $T$
contains a cycle. We first remove all tree-substructures of $G_1$ and
map these as in the proof of \lemref{lem:gd-map-tree}.  Next, we
consider all faces of the remainder of $G_1$ and show how to
iteratively map them.

Consider a cycle $C$ bounding a face $F$ and let $e_1$ and $e_2$ be
two edges of $C$ incident to a vertex $v$. Let $b$ be the line segment
of the bisector of $e_1$ and $e_2$ inside $B_\eps(v)$. We define the
\emph{outermost placement} of $v$ as the placement which intersects
$b$ at maximum distance to the endpoint of $b$ inside $F$, see
Figure~\ref{fig:gd-outer-placement}~(a).  Furthermore, we define an
\emph{outermost path} in $G_2$ of an edge $e=\{u,v\}$ of $G_1$ as the
path $P_{out}$ with maximum distance to $F$ connecting the outermost
placements of $u$ and $v$. That is, no subpath $Q$ of $P_{out}$ can be
replaced by a path $R$ such that $\delta_H(R,B) \leq \delta_H(Q,B)$,
where $\delta_H$ is the Hausdorff distance and $B$ is the boundary of
the tube $T_\eps(e)$ which lies inside the face $F$.  Note that if an
edge is shorter than $2\eps$, and hence the $\eps$-balls around the
vertices overlap, then so possibly do the placements. In particular,
in this case the outer placements may overlap, in which case the edge
placements degenerate, see Figure~\ref{fig:gd-outer-placement}~(a).
Finally, we define an \emph{outer placement} $O$ of $C$ in $G_2$ as
the concatenation of all outermost paths of edges of $C$.

Note that if $C$ is sufficiently convex the outer placement is simply
the cycle that bounds $H$.  See
Figure~\ref{fig:gd-outer-placement}~(b) for an example, where the red
outer placement bounds the outer face of $G_2$ restricted to red and
pink vertices and edges.  The outer placement of $C$ is a weak
$\eps$-placement of $C$.

\begin{figure}
\centering
\subfloat[A vertex with its placement.]{
	\includegraphics[page=1, width=0.2\textwidth]{outerplacement}
	\label{subfig:outer-placement}}
\quad
\subfloat[A cycle with its outer placement.]{
	\includegraphics[page=1, width=0.35\textwidth]{weak-dist-plane}
	\label{subfig:gd-outer-placement}}
\quad
\subfloat[Merging two outer placements.]{
	\includegraphics[page=2, width=0.35\textwidth]{weak-dist-plane}
	\label{subfig:gd-merge-outer-placements}}
\caption{Illustration of outer placements and how to merge them. In (c) %In~\protect\subref{subfig:gd-merge-outer-placements},
the outer placements of cycles $C_1$ and $C_2$ can be merged by mapping the shared path $P$ through~$o_1$.}
\label{fig:gd-outer-placement}
\end{figure}

Now, consider two cycles $C_1$ and $C_2$ bounding adjacent faces of
$G_1$, which share a single (possibly degenerate) path $P$ between
vertices $u$ and $v$.  Let $O_1$ and $O_2$ be the outer placements of
$C_1$ and $C_2$, respectively.  By definition of an outermost
placement, $O_1$ and $O_2$ must intersect inside the intersection of
the $\eps$-tubes of $C_1$ and $C_2$. Let $o_1$ and $o_2$ of $O_1$ and
$O_2$ be the parts between the intersections of $O_1$ and $O_2$
containing the respective images of $P$. Again, by definition of an
outermost placement, it holds that $o_1$ is completely inside $O_2$
and $o_2$ is completely inside $O_1$.

This is illustrated in Figure~\ref{fig:gd-outer-placement}~(c). By
planarity there must be a vertex at the intersections of $O_1$ and
$O_2$. Thus, we can construct a mapping $O'_2$ of $C_2$ that consists
of $o_1$ and $O_2\setminus o_2$.  This is a weak $\eps$-placement of
$C_2$ for which the image of the shared path $P$ is identical to its
image in $O_1$.  Thus, we can merge $O_1$ and $O'_2$ to obtain a weak
$\eps$-placement of these two adjacent cycles.  Note that the mapping
of $C_1$ is not modified in this construction.  Additionally, the
image of the cycle bounding the outer face is its outer placement.
The same argument can be applied iteratively when $C_1$ and $C_2$
share multiple paths.

If there are two cycles $C_1$ and $C_2$ which are connected by a path
$P$ such that one endpoint $u$ of $P$ lies on $C_1$, the other
endpoint $v$ of $P$ lies on $C_2$ and all other vertices of $P$ are no
vertices of $C_1$ or $C_2$, we can still construct a common placement
for $C_1$, $C_2$ and $P$: Let $C_u$, $C_v$ be the outermost placements
of $u$ and $v$, respectively and let $D_v$ be a vaild placement of $v$
which is connected by a path $Q$ in $G_2$ to $C_u$ such that
$\delta_{wF}(Q,P) \leq \eps$. Such a placement $D_v$ must exist as
$C_u$ is a valid placement. If $D_v$ = $C_v$ we have found a common
valid placement for $C_1$, $C_2$ and $P$. If $D_v \neq C_v$, by
definition of an outermost placement, the path $Q$ must intersect the
outermost placement $O$ of $C_2$ inside the intersection of the tubes
$T_\eps(P)$ and $T_\eps(C_2)$. As $G_2$ is plane, there is a vertex
$w$ at the intersection and the resulting path $R=Q_{C_u\rightarrow w}
+ O_{w \rightarrow C_v}$ with $\delta_{wF}(R,P)\leq\eps$ connects
$C_u$ and $C_v$.

Now, we iteratively map the cycles bounding faces of $G_1$ until $G_1$
is completely mapped.  Let $\langle F_1,F_2,\ldots,F_k\rangle$ be an
ordering of the faces of $G_1$ such that each $F_i$, for $i\geq 2$ is
on the outer face of the subgraph $\G_{i-1} := C_1\cup
C_2\cup\ldots\cup C_{i-1}$ of $G_1$, where $C_j$ is the cycle bounding
face $F_j$.  Thus, let $F_1$ be an arbitrary face of $G_1$ and
subsequently choose faces adjacent to what has already been mapped.
Hence when adding a cycle $C_i$, we have already mapped $\G_{i-1}$
such that the cycle bounding its outer face is mapped to its outer
placement.  Thus, we can treat $\G_{i-1}$ as a cycle, ignoring the
part of it inside this cycle, and merge its mapping with $C_i$ using
the procedure described above.  This leaves the mapping of $\G_{i-1}$
unchanged, hence this is still a weak $\eps$-placement of $\G_{i-1}$.
However, the mapping of $C_i$ is now modified to be identical to that
of $\G_{i-1}$ in the parts where they overlap.  Thus, we can merge
these mappings to obtain a weak $\eps$-placement of $\G_i$.  After
mapping $F_k$ we have completely mapped $G_1$.



==> body/pseudometrics.tex <==
Symmetry follows immediately for the undirected distances.  The
directed distances fulfill the triangle inequality because we can
concatenate two maps and use the triangle inequality of $\R^d$: Let
$G_1$, $G_2$ and $G_3$ be three embedded graphs. An edge $e$ of $G_1$
is mapped to a simple path $p$ in $G_2$. The segments of $p$ are again
mapped to a sequence of simple paths in $G_3$. Thus, when
concatenating two maps, one possible mapping maps each edge $e$ of
$G_1$ to a sequence $S$ of simple paths in $G_3$. Note, that $S$ need
not be simple. However, in that case we can instead map $e$ to a
shortest path $\hat{p}$ in $S$ from beginning to end. As
$\delta_{(w)F}(e,\hat{p}) \leq \delta_{(w)F}(e,S)$ for each edge of
$G_1$, we have $\distDir(G_1,G_2)+\distDir(G_2,G_3) \geq
\distDir(G_1,G_3)$ and $\distDirWeak(G_1,G_2)+\distDirWeak(G_2,G_3)
\geq \distDir(G_1,G_3)$ by definition of the directed (weak) graph
distance as the maximum \fr\ of an edge and its mapping.  Analogously,
the undirected distances fulfill the triangle inequality as well.

For plane graphs, their (weak) graph distance is zero iff their
embeddings are the same, hence the distances are metrics.  If the
(weak) graph distance is zero, every edge needs to be mapped to
itself, hence the embeddings are the same.  If on the other hand, the
embeddings are the same, a graph mapping may map every edge to itself
in the embedding.  Since there are no intersections or overlapping
vertices, this mapping is continuous in the target graph, and the
distance is zero.


